Sound and Complete Witnesses for Template-based Verification of LTL Properties on Polynomial Programs

We study the classical problem of verifying programs with respect to formal specifications given in the linear temporal logic (LTL). We first present novel sound and complete witnesses for LTL verification over imperative programs. Our witnesses are applicable to both verification (proving) and refutation (finding bugs) settings. We then consider LTL formulas in which atomic propositions can be polynomial constraints and turn our focus to polynomial arithmetic programs, i.e. programs in which every assignment and guard consists only of polynomial expressions. For this setting, we provide an efficient algorithm to automatically synthesize such LTL witnesses. Our synthesis procedure is both sound and semi-complete. Finally, we present experimental results demonstrating the effectiveness of our approach and that it can handle programs which were beyond the reach of previous state-of-the-art tools.

==> LTL_to_Buchi.tex <==
\section{From LTL to Büchi Specifications}
\label{ltl_to_buchi}

In what follows, we first focus on the ELTL-PA problem and show that it can be reduced to the existential program analysis for Büchi specifications. We will turn our attention to the ULTL-PA problem in Section~\ref{Universal}. Let $\T = (\mathcal{V}, L,  l_\init, \theta_{\init}, \mapsto)$ be a transition system.


%Our main theoretical contribution in this paper is reducing $\LSAT$ to $\BSAT$ and introducing sound and complete ranking function-like witnesses for $\BSAT$. Later, in section \ref{algo}, we give an (\textcolor{red}{?complexity?}) algorithm for finding such witnesses.

\begin{paragraph}{From LTL to Büchi Specifications}
	Denote by $2^S$ the set of all subsets of a set $S$. It is a classical result in model checking that for every LTL formula $\phi$ defined over atomic predicates $AP$ there exists a non-deterministic Büchi automaton $N$ with alphabet $2^{AP}$ which recognizes the same language~\cite{henzinger18}. Recall, a {\em non-deterministic Büchi automaton (NBW)} is an ordered tuple $N=(Q,A,\delta, q_0, F)$, where 
	\begin{compactitem}
		\item $Q$ is a finite set of states,
		\item $A$ is a finite alphabet, 
		\item $\delta\colon Q \times A \to 2^Q$ is a transition relation,
		\item $q_0$ is the initial state, and
		\item $F \subseteq Q$ is the set of accepting states.
	\end{compactitem}
	A run in $N$ is an infinite sequence $q_0,q_1,\dots$ of states in $Q$. A run is accepting if it visits states in $F$ infinitely many times. An infinite word $a_0,a_1,\dots$ of letters in the alphabet $A$ is said to be accepting if it gives rise to at least one accepting run in $N$, i.e.~there exists an accepting run $q_0,q_1,\dots$ such that $q_{i+1} \in \delta(q_i,a_i)$ for each $i$. Finally, the language accepted by $N$, denoted $L(N)$, is the set of all infinite words that are accepting in $N$. Thus, the above result implies that if $\phi$ is an LTL formula over atomic predicates $AP$, then there exists an NBW $N=(Q,2^{AP},\delta, q_0, F)$ such that $L(N)$ is exactly the set of all infinite sequences of elements of $2^{AP}$ that satisfy $\phi$.
\end{paragraph}

\paragraph{From existential LTL to existential Büchi program analysis} We now show that, if $\phi$ is an LTL formula defined over atomic predicates $AP$, then in order to solve the ELTL-PA problem it suffices to solve the EB-PA problem in the transition system obtained by taking the product of $\T$ and the non-deterministic Büchi automaton for the specification $\phi$. We first formally define the notion of a product of a transition system and a non-deterministic Büchi automaton.

In what follows, we assume that $AP$ is a set of finitely many atomic predicates over a transition system $\T$. Recall, we allow atomic predicates in transition systems to either be constraints of the form $\textrm{exp}(\mathbf{x})\geq 0$ or $\at(l)$ for some location $l$ in $\T$. Given a set of atomic predicates $\alpha\in 2^{AP}$, we write $\alpha^{-\mathit{at}} = \alpha \backslash \{\at(l) \mid l\in L\}$ for the set of atomic predicates obtained by removing each $\at(l)$ from $\alpha$.

\begin{definition}[Product of Transition System and Büchi Automaton]
	Let $\T = (\mathcal{V}, L,  l_\init, \theta_{\init}, \mapsto)$ be a transition system and $N = (Q,2^{AP}, \delta, q_0, F)$ an NBW. The {\em product} of $\T$ and $N$ results in a transition system $\T \times N = (\mathcal{V}, L', l_\init', \theta_{\init}, \leadsto)$ and a set of states $\B^\T_N$ in it that are defined as follows:
	\begin{compactitem}
		\item $L'$ is the Cartesian product $L \times Q$.
		\item $l'_\init = (l_\init, q_o)$.
		\item For each transition $\tau=(l,l',G_\tau,U_\tau) \in \,\mapsto$, states $q,q' \in Q$ in $N$ and $\alpha\in 2^{AP}$ such that $q' \in \delta(q,\alpha)$ and $\at(l)\in\alpha$, we include a transition $\big((l,q), (l',q'), G_\tau \wedge \alpha^{-\mathit{at}}, U_\tau \big)$ in $ \leadsto$.
		\item $\B^\T_N = L \times F \times \R^n$, i.e.~$\B^\T_N$  is the set of states in $\T \times N$ whose NBW state component is contained in $F$.
	\end{compactitem}
\end{definition}

%\begin{paragraph}{Büchi Automaton}
%	Recall that a Non-deterministic Büchi Automaton (NBW) is a tuple $N=(Q,A,\delta, q_0, F)$ where 
%\begin{itemize}
%	\item $Q$ is a finite set of states.
%	\item $A$ is the finite set of alphabet. 
%	\item $\delta\colon Q \times A \to \mathcal{P}(Q)$ is a transition relation. 
%	\item $q_0$ is the initial state.
%	\item And $F \subseteq Q$ is the set of accepting states where $N$ accepts exactly those runs that visit $F$ infinite number of times. 
%\end{itemize}
%\end{paragraph}
%The automaton is said to be deterministic if the codomain of $\delta$ contains only singletons.

\begin{example}
	Figure \ref{example_nbw} shows an example Büchi automaton $N$ accepting the runs satisfying $[G\ F\ \at(l_2)]$ with $q_1$ as the only accepting node. On the right side, figure \ref{example_mult} shows the product of the transition system in figure \ref{example_ts} and $N$ with Büchi specification $\B^\T_N$ specified by the gray-scaled locations.
\end{example}

The next theorem is our main result for this section.
\begin{theorem}[Reduction from Existential LTL to Existential Büchi]
	\label{exists_reduction}
	Let $\T$ be a transition system, $\phi$ be an LTL formula for $\T$ and $N$ be an NBW that accepts the same language as $\phi$. Then, there exists a scheduler in $\T$ which solves the ELTL-PA problem for $\T$ and $\phi$ if and only if there exists a scheduler in $\T \times N$ which solves the EB-PA problem for $\T \times N$ and $\B^\T_N$.
\end{theorem}

\begin{proof}
	First, suppose that there exists a scheduler $\sigma$ in $\T$ such that $\pi_\sigma = (l_0, e_0), (l_1, e_1), \dots$ satisfies $\phi$. Let $AP$ be the set of atomic predicates in $\phi$, and for each $i$ let $\alpha_i\in 2^{AP}$ be the set of all atomic predicates that are true in $(l_i,e_i)$. Then, since $N$ accepts the same language as $\phi$, we have that $\alpha_0,\alpha_1,\dots$ is an infinite word in the alphabet $2^{AP}$ which is accepting in $N$. Let $q_0,q_1,\dots$ be an accepting run in $N$ induced by this infinite word, and consider the following sequence of states in $\T \times N$:
	\[
	\pi' = (l_0, q_0, e_0), (l_1, q_1, e_1), \dots
	\]
	We claim that this sequence is a run, i.e.~that $(l_i, q_i, e_i) \leadsto (l_{i+1}, q_{i+1}, e_{i+1})$ for each $i$ where $\leadsto$ is the set of transitions in $\T \times N$. To see this, note that since $\pi_\sigma = (l_0, e_0), (l_1, e_1), \dots$ is a run in $\T$, for each $i$ there exists a transition $\tau=(l_i,l_{i+1},G_\tau,U_\tau)$ under which $(l_{i+1},e_{i+1})$ is a successor of $(l_i,e_i)$. On the other hand, we also know that $q_{i+1}\in \delta(q_i,\alpha_i)$ where $\delta$ is a transition function of $N$. Finally, since $\alpha_i$ is the set of all atomic predicates in $AP$ that are true at $(l_i,e_i)$, we must have $\at(l_i)\in\alpha_i$. Hence, we have that $(l_i, q_i, e_i) \leadsto (l_{i+1}, q_{i+1}, e_{i+1})$ under transition $((l_i,q_i),(l_{i+1},q_{i+1}),G_\tau\land \alpha^{-\at},U_\tau)$ and the claim follows. Finally, since $q_0,q_1,\dots$ is accepting in $N$ we have that $\pi' = (l_0, q_0, e_0), (l_1, q_1, e_1), \dots$ contains infinitely many states in $\B^\T_N$, Hence, taking a scheduler in $\T \times N$ which induces the run $\pi'$ solves the EB-PA problem for $\T \times N$ and $\B^\T_N$. 
	
	For the opposite direction, suppose that there exists a scheduler in $\T \times N$ which yields a run $\pi' = (l_0, q_0, e_0), (l_1, q_1, e_1), \dots$ that visits $\B^\T_N$ infinitely many times. The definition of transitions in the product transition system $\T \times N$ implies that $(l_0, e_0), (l_1, e_1), ...$ is a run in $\T$, that $q_0,q_1,\dots$ is an accepting run in $N$ and that there exists an infinite accepting word $\alpha_0,\alpha_1,\dots$ in $2^{AP}$ such that $\at(l_i) \in \alpha_i$ for each $i$. Since $\alpha_0,\alpha_1,\dots$ is accepting in $N$ and $\at(l_i) \in \alpha_i$ for each $i$ and since $N$ and $\phi$ accept the same languages, it follows that $(l_0, e_0), (l_1, e_1), ...$ satisfies $\phi$. Hence, taking a scheduler in $\T$ which induces the run $(l_0, e_0), (l_1, e_1), ...$ solves the ELTL-PA problem for $\T$ and $\phi$. \hfill\qed
\end{proof}

%\begin{proof}
%	Let $\sigma$ be a scheduler for $\T$ where $\pi_\sigma = [(l_0, e_0), (l_1, e_1), \dots]$ satisfies $\phi$. As illustrated earlier, this is equivalent to $\pi_\sigma$ being accepted by $N$. Suppose $r = [q_0, a_0, q_1, a_1, \dots]$ is the run in $N$ accepting $\pi_\sigma$. Then it is easy to see that the following run in $\T \times N$ is $\B^\T_N$-Büchi:
%	\[
%	\pi' = [ (l_0, q_0, e_0), (l_1, q_1, e_1), \dots ]
%	\]
%	The reverse is true by similar arguments: If $\pi'$ is a $\B^\T_N$-Büchi run in $\T \times N$, then the run $r$ is accepted by $N$ which shows that $\pi_\sigma$ satisfies $\phi$. Existence of $\sigma$ is trivial. This completes the proof.
%\end{proof}

Theorem~\ref{exists_reduction} implies that, instead of searching for witnesses for solving the ELTL-PA problem, in what follows it will suffice to construct the product transition system as above and to search for witnesses for solving the EB-PA problem.

\input{example_mult}

%For the universal problem, the case is a bit different because an NBW has an existential quantification in its acceptance condition. The universal quantifier in the definition of universal LTL together the existential quantifier in the semantics of the NBW would create undefinable situations for the non-deterministic characteristics of the product transition system. Therefore, for universal LTL checking, we restrict the LTL formula to have an equivalent deterministic Büchi automaton (DBW). This way, an infinite word $w$ is accepted by the automaton $D$ if and only if the unique path corresponding to $w$ is accepting $D$.

%Although DBWs are strictly less expressive than NBWs, there has been a lot of research on algorithms for constructing a DBW given an NBW, if possible \cite{schulte06, henzinger18}. Moreover, many of the LTL formulae used in the literature for verifying various properties have deterministic Büchi automaton counterparts.

%\begin{theorem}[Reduction from Universal LTL to Universal Büchi]
%	Let $\T$ be a transition system and $\phi$ be an LTL formula on $\T$ which is equivalent to DBW $D$. The universal LTL checking of $\T$ and $\phi$ is equivalent to universal Büchiness problem of $\T \times D$ and $\B^\T_D$.
%\end{theorem}

%\begin{proof}
%	Suppose every run $\pi \in \Pi$ satisfies $\phi$ or equivalently that every run $\pi \in \Pi$ is accepted by $D$. For the sake of contradiction, let $[(s_0, q_0, e_0), (s_1,q_1,e_1), \dots]$ be a run in $\T \times D$ which is not $B^\T_D$-Büchi. This would mean that the run $[q_0, q_1, \dots]$ is not accepting in $D$, therefore $D$ does not accept $[(s_0,e_0), (s_1,e_1) \dots]$ which is a contradiction.
	
%	For the reverse, suppose every run in $\T \times D$ is $\B^\T_D$-Büchi and for the sake of contradiction let $\pi = [(s_0,e_0), \dots ]$ be a run in $\T$ which does not satisfy $\phi$, or equivalently, is not accepted by $D$. Therefore, the run $[(s_0, q_0, e_0), \dots]$ is not $\B^\T_D$-Büchi which means $[q_0, q_1, \dots]$ is not accepting in $D$ resulting a contradiction. 
%\end{proof}


==> Memory-lemmas.tex <==
\subsection{Sufficiency of Memory-Less Schedulers }

The goal of this section is to show that existence of memory-less schedulers that generate $\B$-Büchi runs is equivalent to existence of generic (history dependent) schedulers that generate $\B$-Büchi runs. We start by defining the cycle-decomposition of a trajectory. Recall that trajectories are finite sub-sequences of runs and cycles are trajectories starting and ending in the same state.

\begin{definition}[Cycle-Decomposition of a Trajectory]
	For a trajectory $\tau$ starting at $s_1$ and ending at $s_2$, we define its Cycle-Decomposition as a tuple $(C, \beta)$ where $C$ is the set of all cycles appearing as a sub-trajectory of $\tau$ and $\beta$ is the underlying non-cyclic trajectory in $\tau$ going from $s_1$ to $s_2$.  See figure \ref{cycle-dec-example} for an example.
\end{definition}

\input{example-cy-dec}

In order to construct the cycle-decomposition $(C,\beta)$ of $\tau$, we go through $\tau$ and push the states one by one into a stack. Whenever we visit a state $s$ already in the stack, we pop all the elements between the two occurrences of $s$ (including only one of the occurrences) and add them as a cycle to $C$. Finally, $\beta$ will be the trajectory constructed by the states remaining in the stack at the end.

As our witness corresponds to memory-less schedulers, in order to prove completeness we need to show that existence of a memory-less scheduler that corresponds to a $\B$-Büchi run is in fact, equivalent to existence of a $\B$-Büchi generic scheduler. The following theorem demonstrates this. 

\begin{lemma}
	\label{mem-angelic}
	There exists a memory-less $\B$-Büchi scheduler for $\T$, if and only if, there exists a $\B$-Büchi scheduler for $\T$. 
\end{lemma}
\begin{proof}
	Necessity is trivial. For sufficiency, suppose $\sigma$ is a $\B$-Büchi scheduler. We construct a memory-less scheduler $\sigma'$ based on $\sigma$. 
	
	Let $\pi = \pi_\sigma$ and let $(C_i, \beta_i)$ be the cycle-decomposition of $\pi^i$ for all $i \geq 0$. One of the following cases can happen:
	\begin{enumerate}[(i)]
		\item $\pi$ has no cycles. In this case, $\sigma$ was not using the history of the run to generate $\pi$. Therefore, we can define $\sigma'$ to be the same as $\sigma$ on $\pi$ and arbitrary on other states. $\pi_{\sigma'}$ will then be the same as $\pi_\sigma$ proving that $\sigma$ is $\B$-Büchi. 
		\item $\pi$ has finite number of cycles. So, there exists $k$ such that $\pi^{k+}$ is non-cyclic which means $\beta_k \cdot \pi^{k+}$ is a $\B$-Büchi run with no cycles where we can apply case (i).
		\item $\pi$ has infinite number of cycles. Here we would have two sub-cases:
		\begin{itemize}
			\item $\pi$ contains a cycle $c$ starting at $\pi(b)$ which intersects with $\B$. Let $k$ be the smallest index where $\pi(k) = \pi(b)$, then the run $\pi' = \beta_k \cdot c^\omega$ is easily seen to be $\B$-Büchi. As each state in $\pi'$ has a unique successor in the run, there exists a memory-less scheduler $\sigma'$ where $\pi_{\sigma'} = \pi'$.
			\item None of the cycles of $\pi$ intersect with $\B$. Removing all cycles from $\pi$ produces a non-cyclic $\B$-Büchi run $\pi'$. The rest was handled in case (i).
		\end{itemize}
	\end{enumerate}\hfill\qed
\end{proof}

Intuitively, lemma \ref{mem-angelic} shows that memory-less schedulers are just as powerful as general schedulers when it comes to Büchi or (as stated in section \ref{decision_problems}) LTL specifications. 

==> Overview.tex <==
\section{Overview}

==> Universal.tex <==



==> exp_results_table.tex <==
\begin{table}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Formula} & \multicolumn{3}{c|}{Ours} & \multicolumn{3}{c|}{Ultimate} & \multicolumn{3}{c|}{nuXmv} & \multicolumn{3}{c|}{Z3 SMT Solver}\\
		\cline{2-13}
		& Yes & No & Unique & Yes & No & Unique & Yes & No & Unique & Yes & No & Unique \\
		\hline
		$RA$ & 140 & 113 & 11 & 142 & 116 & 12 & 76 & 91 & 2 & 56 & 36 & 0 \\
		%\hline 
		%$RA_2$ & 94 & 114 & 11 & 96 & 152 & 27 & 44 & 96 & 6 & 31 & 34 & 0 \\
		\hline 
		$OV$ & 199 & 47 & 8 & 211 & 55 & 17 & 110 & 50 & 3 & 48 & 27 & 0\\
		\hline 
		$PR$ & 87 & 192 & 1 & 87 & 194 & 0 & 80 & 184 & 0 & 40 & 95 & 0 \\
		\hline
	\end{tabular}
	\caption{Experimental Results on Linear Benchmarks}
	\label{experiments_results_linear}
\end{table}

\begin{table}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Benchmark} & \multicolumn{3}{c|}{Ours} & \multicolumn{3}{c|}{nuXmv}\\
		\cline{2-7}
		& $RA$ & $OV$ & $PR$ & $RA_1$ & $OV$ & $PR$\\
		\hline
		\makecell{\texttt{ChawdharyCookGulwaniSagivYang-ESOP}\\\texttt{2008-aaron12_true-termination.c}} & \checkmark & \checkmark & - & - & - & - \\
		\hline
		\texttt{ComplInterv.c} & \xmark & \checkmark & \xmark & - & - & \xmark \\
		\hline
		\texttt{DoubleNeg.c} & \checkmark & \checkmark & \xmark & - & - & -\\
		\hline
		\texttt{Factorial.c} & \xmark & - & \checkmark & - & \checkmark & -\\
		\hline
		\texttt{LogMult.c} & \checkmark & \checkmark & \checkmark & - & - & -\\
		\hline
		\texttt{svcomp_ex1.c} & \checkmark & \checkmark & - & - & \checkmark & \xmark\\
		\hline
		\texttt{svcomp_ex2.c} & - & \checkmark & \checkmark & - & \checkmark & \checkmark\\
		\hline
		\texttt{svcomp_ex3a.c} & \checkmark & \checkmark & \checkmark & - & - & -\\
		\hline
		\texttt{svcomp_ex3b.c} & \checkmark & \checkmark & \checkmark & - & - & -\\
		\hline
		\texttt{svcomp_fermat.c} & \checkmark & \checkmark & \checkmark & - & - & -\\
		\hline
		\hline 
		Total Proved & 9 & 9 & 8 & 0 & 3 & 3 \\
		\hline
	\end{tabular}
	\caption{Experimental Results on Polynomial Benchmarks. \checkmark~is used whenever the formula is universally proved on the benchmark and \xmark~when the formula is existentially disproved.}
	\label{experiments_results_poly}
\end{table}

==> exp_smt_table.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{|c||c|c||c|c||c|c|}
		\hline
		\multirow{2}{*}{Formula} & \multicolumn{2}{c||}{Barcelogic}  & \multicolumn{2}{c||}{MathSAT5} & \multicolumn{2}{c|}{Z3}\\
		\cline{2-7}
		& Yes & No & Yes & No & Yes & No\\
		\hline
		$RA$ & 115 & 91 & 138 & 106 & 81 & 42 \\
		%\hline
		%$RA_2$ & 62 & 66 & 93 & 111 & 43 & 23 \\
		\hline
		$OV$ & 138 & 38 & 197 & 46 & 111 & 28 \\
		\hline
		$PR$ & 75 & 139 & 84 & 189 & 39 & 109 \\
		\hline
	\end{tabular}
	\caption{Performance of our Approach using Different SMT Solvers}
	\label{experiments_separated}
\end{table}

==> motivatingexamples.tex <==
\section{Motivating Examples for LTL Program Analysis}\label{sec:motivatingexamples}

\def\bluecolor{\color{blue}}
\def\blackcolor{\color{black}}

In this work, we consider two variants of LTL program analysis: \emph{Universal} analysis asks whether \emph{every run} of a given program satisfies a given LTL specification $\varphi,$ whereas \emph{existential} analysis aims to decide if \emph{there exist} a run satisfying $\varphi.$ We illustrate these variants on two motivating examples. Both examples consider pairs of programs with non-determinism and LTL specifications whose satisfaction we wish to analyze. For each program pair, only some (but not all) runs of the first program satisfy the LTL specification, whereas all runs of the second program satisfy the LTL specification. Moreover, in both examples, we consider LTL specifications that cannot be reduced to termination, reachability or safety. Thus, the goal in each of these examples cannot be simply reduced to termination, reachability or safety analysis and hence, previous approaches for these classical problems are inapplicable here. In other words, LTL specifications not only generalize safety, liveness, termination and reachability, but are also strictly more expressive.

%We start by presenting our two examples. The first example considers an instance of what are commonly referred to as {\em reach-avoid specifications} in program analysis and formal methods literature. The second example considers an instance of what are commonly referd to as {\em progress specifications}.

\begin{example}[Reach-avoid specifications]
	Our first example program pair illustrates the Existential and Universal LTL Program Analyses for {\em reach-avoid specifications}. Intuitively, a run is said to satisfy a reach-avoid  specification if it reaches some ``target'' set of program states while avoiding some ``unsafe'' set of program states. A common scenario in which reach-avoid specifications arise in program analysis is if we require all runs in a program to terminate while satisfying all assertions specified by the programmer. This example illustrates one such scenario. Reach-avoid specifications are also extremely common in the analysis of dynamical or hybrid systems~\cite{reach-avoid1,reach-avoid2,ZikelicLHC23}.
	
	Consider the program pair shown in Figure~\ref{fig:motivatingone}. Both programs initialize variable $i$ to $1$, variable $s$ to $0$, and consist of a loop that is executed as long as $i \leq n$. In each loop iteration, the programs may or may not increment the value of $s$ by $i$. Whether $s$ is incremented or not is subject to a non-deterministic choice, indicated in the program syntax by a command \textbf{if $\ast$ then}. At the end of each loop iteration, in both programs $i$ is incremented by $1$. The two programs only differ in the assertion by which they are annotated. The program on the left is annotated by \textbf{assert}($s \leq n(n-1)/2$) at the location $l_1$ of the loop head, whereas the program on the right is annotated by \textbf{assert}($s \leq n(n+1)/2$) at the same location. Assertions in both programs are highlighted in blue.
	
	In both programs, a run satisfies the reach-avoid specification if it terminates (i.e.~reaches $l_t$) while satisfying assertions in all visited program locations. This specification for programs in Figure~\ref{fig:motivatingone} left and right is formalized via the following LTL formulas:
	\begin{equation*}
	\begin{split}
		\phi_{\text{left}} &= \Big[\Big(\F\ \at(l_t) \Big) \land \Big(\G\ (\at(l_1) \Rightarrow s \leq n \cdot (n-1)/2)\Big)\Big], \\
		\phi_{\text{right}} &= \Big[\Big(\F\ \at(l_t)\Big) \land \Big(\G\ (\at(l_1) \Rightarrow s \leq n \cdot (n+1)/2)\Big)\Big],
	\end{split}
	\end{equation*}
	where we use $\at(l)$ to denote the atomic proposition that a program run is in location $l$. We will formalize the syntax and semantics of LTL in Section~\ref{prelim}. The two specifications are different due to different assertions by which the two programs in Figure~\ref{fig:motivatingone} are annotated.

\begin{figure}[t]
	\centering
	\begin{subfigure}{0.47\textwidth}
		\begin{lstlisting}[frame=none,numbers=none,escapechar=@]
Precondition$(l_{init})$:$\,n \geq 1,i = 1,s = 0$
$l_1$:  while $i \leq n$ do
      @\aftergroup\bluecolor@assert($s \leq n \cdot (n-1)/2$)@\aftergroup\blackcolor@
      if $\ast$ then
$l_2$:          $s = s + i$
      else 
$l_3$:          skip
      fi
   done
$l_t$:

LTL specification:
$\Big(\F\ \at(l_t) \Big) \land \Big(\G\ (\at(l_1) \Rightarrow s \leq n \cdot (n-1)/2)\Big)$
		\end{lstlisting}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.47\textwidth}
		\begin{lstlisting}[frame=none,numbers=none,escapechar=@]
Precondition$(l_{init})$:$\,n \geq 1,i = 1,s = 0$
$l_1$:  while $i \leq n$ do
     @\aftergroup\bluecolor@assert($s \leq n \cdot (n+1)/2$)@\aftergroup\blackcolor@
     if $\ast$ then
$l_2$:          $s = s + i$
     else 
$l_3$:          skip
     fi
   done
$l_t$:

LTL specification:
$\Big(\F\ \at(l_t)\Big) \land \Big(\G\ (\at(l_1) \Rightarrow s \leq n \cdot (n+1)/2)\Big)$
\end{lstlisting}
		\end{subfigure}
	% \vspace{-1em}
		\caption{Our motivating example program pair for Existential and Universal LTL Program Analysis with reach-avoid specifications. The reach-avoid specification requires that every run in the program terminates while satisfying all assertions shown in blue. Only some (but not all) runs of the program in the left satisfy the reach-avoid specification. In contrast, all runs of the program in the right satisfy the reach-avoid specification.}
	% \vspace{-1em}
		\label{fig:motivatingone}
\end{figure}

Note that all runs of the program in Figure~\ref{fig:motivatingone} (right) satisfy $\phi_{\text{right}}$, whereas only some runs of the program in Figure~\ref{fig:motivatingone} (left) satisfy $\phi_{\text{left}}$. %Indeed, the run which always takes the else-branch of the non-deterministic choice never increments $s$, hence the value of $s$ is equal to $0$ along this run for any initial value of $n$.
Indeed, the value of $s$ along a run is maximized if the run always takes the then-branch of the non-deterministic choice, resulting in the value $\sum_{i=1}^n i = n \cdot (n+1)/2$ upon termination. This run violates the assertion in the program in Figure~\ref{fig:motivatingone} (left) and therefore it violates $\phi_{\text{left}}$. On the other hand, all runs satisfy the assertion in the program in Figure~\ref{fig:motivatingone} (right) and also satisfy $\phi_{\text{right}}$.
%Hence, all runs satisfy the assertion in the program in Figure~\ref{fig:motivatingone} right, whereas only some runs satisfy the assertion in the program in Figure~\ref{fig:motivatingone} left.

The goal of the Universal LTL Program Analysis for this example is to show that {\em all runs} of the program in Figure~\ref{fig:motivatingone} (right) satisfy $\phi_{\text{right}}$. On the other hand, the goal of the Existential LTL Program Analysis is to show that {\em not all runs} of the program in Figure~\ref{fig:motivatingone} (left) satisfy $\phi_{\text{left}}$. The latter is achieved by using the Existential LTL Program Analysis to analyze the negated LTL specification
\begin{equation*}
	\neg\phi_{\text{left}} = \Big[\Big(\G\ \neg\at(l_t)\Big) \lor \Big(\F\ (\at(l_1) \land s > n \cdot (n-1)/2)\Big)\Big].
\end{equation*}
Hence, the Universal LTL Program Analysis {\em \bf proves} a reach-avoid specification for all runs, whereas the Existential LTL Program Analysis {\em \bf refutes} a reach-avoid specification for some run.
\end{example}

\begin{figure}[t]
	\centering
	\begin{subfigure}{0.45\textwidth}
		\begin{lstlisting}[frame=none,numbers=none,escapechar=@]
Precondition$(l_{init})$:$\,n = 100,x = 0,y = 0$
$l_1$: while true do
      $n = 100$
      $x = 1$
      if $\ast$ then
            $y = -1$
      elif $\ast$ then
            $y = 0$
      else
            $y = 1$
      fi

$l_2$:     while $n>0$ do
            $n = n-y$
      done
$l_3$:     $x = 0$
   done
$l_t$:

LTL specification:
$\G\ \Big(x = 1 \Rightarrow (\F\ x = 0)\Big)$
		\end{lstlisting}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.5\textwidth}
		\begin{lstlisting}[frame=none,numbers=none,escapechar=@]
Precondition$(l_{init})$:$\,n = 100,x = 0,y = 0$
$l_1$: while true do
      $n = 100$
      $x = 1$
      if $\ast$ then
            $y = -1$
      elif $\ast$ then
            $y = 0$
      else
            $y = 1$
      fi
$l_2$:     @\aftergroup\bluecolor@assume($y \geq 1$)@\aftergroup\blackcolor@
$l_3$:     while $n>0$ do
            $n = n-y$
      done
$l_4$:     $x = 0$
   done
$l_t$:

LTL specification:
$\Big(\G\ (\at(l_2) \Rightarrow y \geq 1)\Big) \Rightarrow \Big(\G\ (x = 1 \Rightarrow (\F\ x = 0))\Big)$
		\end{lstlisting}
	\end{subfigure}
% \vspace{-1em}
	\caption{Our motivating example program pair for Existential and Universal LTL Program Analysis with progress specifications. The progress specification requires that if a run satisfies all assume statements shown in blue, whenever the run reaches a program state with $x=1$, it must also subsequently reach a program state with $x=0$. Only some (but not all) runs of the program in the left satisfy the progress specification. In contrast, all runs of the program in the right satisfy the progress specification.}
	% \vspace{-1em}
	\label{fig:motivatingtwo}
\end{figure}

\begin{example}[Progress specifications]
	Our second example program pair illustrates the Existential and Universal LTL Program Analyses for {\em progress specifications}. Progress specifications are a subclass of liveness specifications. Intuitively, given two sets of program states $A$ and $B$, a run is said to satisfy the progress specification for $A$ and $B$ if whenever the run reaches a state in $A$ it must also subsequently reach a state in $B$~\cite{0077033}. Examples of progress specifications include starvation freedom, fairness or recurrence~\cite{katoen08}. For our example, we consider a variant of the program and the progress specification in Section 2 of~\cite{CookK13} with finite non-determinism.
	
	Consider the program pair shown in Figure~\ref{fig:motivatingtwo}. Both programs initialize variable $n$ to $100$, variables $x$ and $y$ to $0$, and consist of a loop that is executed indefinitely. In each loop iteration, both programs first set the value of $x$ to $1$. They then non-deterministically choose a value from the set $\{-1,0,1\}$ and assign it to $y$. Then, both programs execute an inner loop that decrements $n$ by $y$ as long as $n>0$. Finally, upon inner loop termination, both programs set the value of $x$ to $0$. The only difference between the two programs is that the program in Figure~\ref{fig:motivatingtwo} (right) is also annotated by an assumption \textbf{assume}($y \geq 1$) at the location $l_2$ before entering the inner loop. The assumption in the program is highlighted in blue.
	
	As in~\cite{CookK13}, we consider the progress specification for sets of states in which $x=1$ and in which $x=0$. In other words, a run satisfies the specification if it either violates some assumption in the program, or if whenever it reaches a state in which $x=1$ it must also subsequently reach a state in which $x=0$. This specification for programs in Figure~\ref{fig:motivatingtwo} is formalized via the following LTL formulas:
	\begin{equation*}
		\begin{split}
			\phi_{\text{left}} &= \Big[\G\ \Big(x = 1 \Rightarrow (\F\ x = 0)\Big)\Big], \\
			\phi_{\text{right}} &= \Big[\Big(\G\ (\at(l_2) \Rightarrow y \geq 1)\Big) \Rightarrow \Big(\G\ (x = 1 \Rightarrow (\F\ x = 0))\Big)\Big].
		\end{split}
	\end{equation*}

	Note that all runs of the program in Figure~\ref{fig:motivatingtwo} (right) satisfy $\phi_{\text{right}}$. Indeed, if a run satisfies all assume statements, then the program must assign $y=1$ in every outer loop iteration. This means that the inner loop must always terminate as each inner loop iteration decrements $n$ by $1$, therefore the run reaches a state with $x=0$ infinitely many times. On the other hand, only some runs of the program in Figure~\ref{fig:motivatingtwo} (left) satisfy $\phi_{\text{left}}$. %Indeed, the run which always assigns $y=1$ satisfies the specification. However,
	Any run which in some outer loop iteration assigns $y=-1$ or $y=0$ enters the inner loop that never terminates since $n$ is never decremented, so the value of $x$ is $1$ indefinitely.
	
	The goal of the Universal LTL Program Analysis for this example is to show that {\em all runs} of the program in Figure~\ref{fig:motivatingone} (right) satisfy $\phi_{\text{right}}$. On the other hand, the goal of the Existential LTL Program Analysis is to show that {\em not all runs} of the program in Figure~\ref{fig:motivatingone} (left) satisfy $\phi_{\text{left}}$. The latter is achieved by using the Existential LTL Program Analysis to analyze the negated LTL specification
	%Our method for the Universal LTL Program Analysis automatically shows that {\em all runs} of the program in Figure~\ref{fig:motivatingtwo} (right) satisfy $\phi_{\text{right}}$. On the other hand, our method for the Existential LTL Program Analysis shows that {\em not all runs} of the program in Figure~\ref{fig:motivatingtwo} (left) satisfy $\phi_{\text{left}}$. The latter is achieved by using our method for the Existential LTL Program Analysis to analyze the negated LTL specification
	\begin{equation*}
		\neg\phi_{\text{left}} =  \Big[\F\ \Big( x = 1 \land \G\ x \neq 0 \Big)\Big].
	\end{equation*}
	Hence, the Universal LTL Program Analysis {\em \bf proves} a progress specification for all runs, whereas the Existential LTL Program Analysis {\em \bf refutes} a progress specification for some run.
	%Hence, our method for LTL program analysis is able both {\em to prove} and {\em to refute} the satisfaction of a progress specification in a program.
\end{example}

The above examples highlight the importance of analysis of non-linear programs with respect to specifications described as LTL formulas,
which are beyond safety and termination properties. 
This is precisely the focus of the current work.
